Dynamic Hierarchical $j$-Tree Decomposition and Its Applications

We develop a new algorithmic framework for designing approximation algorithms for cut-based optimization problems on capacitated undirected graphs that undergo edge insertions and deletions. Specifically, our framework dynamically maintains a variant of the hierarchical $j$-tree decomposition of [Madry FOCS'10], achieving a poly-logarithmic approximation factor to the graph's cut structure and supporting edge updates in $O(n^{\epsilon})$ amortized update time, for any arbitrarily small constant $\epsilon \in (0,1)$. Consequently, we obtain new trade-offs between approximation and update/query time for fundamental cut-based optimization problems in the fully dynamic setting, including all-pairs minimum cuts, sparsest cut, multi-way cut, and multi-cut. For the last three problems, these trade-offs give the first fully-dynamic algorithms achieving poly-logarithmic approximation in sub-linear time per operation. The main technical ingredient behind our dynamic hierarchy is a dynamic cut-sparsifier algorithm that can handle vertex splits with low recourse. This is achieved by white-boxing the dynamic cut sparsifier construction of [Abraham et al. FOCS'16], based on forest packing, together with new structural insights about the maintenance of these forests under vertex splits. Given the versatility of cut sparsification in both the static and dynamic graph algorithms literature, we believe this construction may be of independent interest.

==> contents/references.tex <==
\clearpage
%\pagenumbering{arabic}
%
%\renewcommand{\thepage}{References - \arabic{page}}


\section*{References}
\printbibliography[heading=none]

\clearpage

==> template/biblatex-setup.tex <==
\usepackage{listings}
\lstset{
  literate={ö}{{\"o}}1
           {ä}{{\"a}}1
           {ü}{{\"u}}1
}


\usepackage[
    backend=bibtex,    %% Backend for processing
    maxcitenames=10,    %% Maximum names in citations
    maxbibnames=10,    %% Maximum names in entries
%    maxsortnames=10,    %% Limit sorting
    maxalphanames=10,    
    maxnames=10,    %% Limit total names in citations
    style=alphabetic,    %% Citation style
    sorting=anyt,    %% Sort entries by author/title/year
    doi=false,    %% DOI in bibliography
    isbn=false,    %% ISBN in bibliography
    eprint=false,    %% Eprint in bibliography
    url=false,    %% URL in bibliography
	backref=true,    %% Back-referencing to pages
	backrefstyle=none,    %% Back-reference style
        ]{biblatex}


\AtEveryBibitem{
\ifentrytype{inproceedings}{
\clearname{editor}%
\clearfield{valume}%
\clearfield{number}%
\clearfield{series}%
\clearlist{publisher}%
\clearfield{address}%
\clearlist{location}%
\clearfield{month}%
\clearfield{eprint}%
\clearfield{isbn}%
\clearfield{issn}%
}{}
}


%% Combine the doi link with the entries' title
\newbibmacro{string+doi}[1]{%
    \iffieldundef{doi}{%
        \iffieldundef{url}{#1}{\href{\thefield{url}}{#1}}
        }{%
        \href{http://dx.doi.org/\thefield{doi}}{#1}
        }
    }

\DeclareFieldFormat*{title}{%
    \usebibmacro{string+doi}{\mkbibemph{#1}}
    }

%% "In:" removed for articles; issue/date macros added after note+pages macro
\renewbibmacro{in:}{%
    \ifentrytype{article}{}{\printtext{\bibstring{in}\intitlepunct}}}
%\renewbibmacro{in:}{}

%% Move year to the end of the bibliographies
\newtoggle{bbx:datemissing}

\renewbibmacro*{date}{\toggletrue{bbx:datemissing}%
}

\renewbibmacro*{issue+date}{}% 

\newbibmacro*{date:print}{%
    \setunit{\addcomma\addspace}    % add comma before year
    \togglefalse{bbx:datemissing}%
    \printdate}

\renewbibmacro*{chapter+pages}{%
    \printfield{chapter}%
    \setunit{\bibpagespunct}%
    \printfield{pages}%
    \newunit
    \usebibmacro{date:print}%
    \newunit}

\renewbibmacro*{note+pages}{% 
    \printfield{note}%
    \setunit{\bibpagespunct}%
    \printfield{pages}%
    \setunit{\addcomma\addspace}%      %  NEW
    \usebibmacro{date}%                %  NEW
    \newunit}

\renewbibmacro*{addendum+pubstate}{%
    \iftoggle{bbx:datemissing}
        {\usebibmacro{date:print}}
        {}%
    \printfield{addendum}%
    \newunit\newblock
    \printfield{pubstate}}


%% Clear the 'pages' field for every entry
%\AtEveryBibitem{\clearfield{pages}} 

%% For entries to respect the margins
\appto{\bibsetup}{\sloppy}

%% Use page(s) instead of p. or pp.
\DefineBibliographyStrings{english}{%
    page={page},%
    pages={pages},%
    }

%% Use "cited on page(s)" for the backref
\DefineBibliographyStrings{english}{
  backrefpage = {},
  backrefpages = {},
}


\renewcommand*{\bibpagerefpunct}{%
  \finentrypunct\space}

\DeclareFieldFormat{bracketswithperiod}{\mkbibbrackets{#1}}

\renewbibmacro*{pageref}{%
  \iflistundef{pageref}
    {}
    {\printtext[bracketswithperiod]{%
       \ifnumgreater{\value{pageref}}{1}
         {\bibstring{backrefpages}}
         {\bibstring{backrefpage}}%
       \printlist[pageref][-\value{listtotal}]{pageref}}%
     \renewcommand*{\finentrypunct}{}}}


\addbibresource{references.bib}
%\renewcommand*{\bibfont}{\footnotesize}
%\AtEveryBibitem{\clearfield{pages}} 

%% Redefine the bibliography font size
\renewcommand*{\bibfont}{\footnotesize}





\newcommand{\FOCS}{FOCS}
\newcommand{\STOC}{STOC}
\newcommand{\SODA}{SODA}
\newcommand{\ICALP}{ICALP}
\newcommand{\KDD}{KDD}
\newcommand{\ITCS}{ITCS}
\newcommand{\ICLR}{ICLR}
\newcommand{\ESA}{ESA}
\newcommand{\NeurIPS}{NeurIPS}
\newcommand{\ICML}{ICML}
\newcommand{\WG}{WG}
\newcommand{\SPAA}{SPAA}
\newcommand{\SOSA}{SOSA}




==> template/body-ref.tex <==
\usepackage{xurl}

\usepackage[
    breaklinks=true,    %% Links can break across lines
    colorlinks=true,    %% Colored links instead of boxes
    linkcolor=myDarkBlue,    %% Color for internal links
    urlcolor=myRed,    %% Color for URLs
    citecolor=myGreen,    %% Color for citation links
    bookmarks=true,    %% Enable PDF bookmarks
    bookmarksopenlevel=2,    %% Expand bookmark level
    ]{hyperref}

%\hypersetup{breaklinks=true}

%\usepackage{url}
%\usepackage[hyphenbreaks]{breakurl}


\usepackage[nameinlink]{cleveref}


\crefname{problem}{problem}{problems}
\crefname{claim}{claim}{claims}
\crefname{lemma}{lemma}{lemmas}
\crefname{algorithm}{algorithm}{algorithms}
\crefname{proof}{proof}{proofs}
\crefname{observation}{observation}{observations}
\crefname{invariant}{invariant}{invariants}


==> template/font.tex <==
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage{microtype}

==> template/margins.tex <==
\usepackage[margin=1in]{geometry}

%\usepackage{mdframed,lipsum}
%\newmdenv[
%%  leftmargin = -10pt,
%  innerleftmargin = 1em,
%  innertopmargin = 0pt,
%  innerbottommargin = 5pt,
%  innerrightmargin = 1em,
%  rightmargin = -10pt,
%  linewidth = 1pt,
%  linecolor = lightgray,
%  topline = false,
%  rightline = false,
%  bottomline = true,
%%  roundcorner= 10pt,
%  ]{leftbar}


%\usepackage{a4wide}


%% Control list spacing
\usepackage{enumitem}
% \setlist{nosep}
% \setlist{noitemsep}
% \setitemize{itemsep=10pt}
% \setenumerate{itemsep=10pt}
% \setlist{labelsep=.25em}
\setlist[itemize]{itemsep=.1pt, topsep=3pt,}
%    leftmargin=*}
\setlist[enumerate]{itemsep=.5pt, topsep=3pt,
    leftmargin=*}




\usepackage{titlesec}

%% use \medbreak to end a paragraph
\titlespacing{\paragraph}{%
  0pt}{%left margin
  1em}{%space before (vertical)
  1em}%space after (horizontal)


\renewcommand\labelitemi{\textbf{--}}



==> template/math.tex <==
\usepackage{amsmath}
\usepackage{amsthm}  % For environments
\usepackage{amssymb}  % For \square symbol
\usepackage{mathtools}
\usepackage{enumitem}
\usepackage[]{bbold}
\usepackage{ntheorem} % For automatic \qedhere

\usepackage{thmtools}
\usepackage{thm-restate}

%\declaretheorem[shaded={bgcolor=myLightBlue!50,
%textwidth=\textwidth}]{theorem}






\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}{Fact}[subsection]
\newtheorem{invariant}{Invariant}[section]

\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}



%%Sample:
%\begin{restatable}{theorem}{main} \label{th:main}
%
%\end{restatable}
%
%\main*






==> template/preamble.tex <==
\input{./template/graphics.tex}
\input{./template/colorscheme.tex}
\input{./template/margins.tex}
\input{./template/math.tex}
\input{./template/algorithm.tex}
\input{./template/macros.tex}
\input{./template/biblatex-setup.tex}
\input{./template/body-ref.tex}
\input{./template/font.tex}
%\input{./template/submission-draft.tex}



==> template/submission-draft.tex <==




\usepackage[displaymath, mathlines]{lineno}
\linenumbers



\expandafter\let\expandafter\oldequation\csname equation*\endcsname
\expandafter\let\expandafter\endoldequation\csname endequation*\endcsname

\def\lneq{\linenomath\oldequation}
\def\endlneq{\endoldequation\endlinenomath}
\renewenvironment{equation*}{%
  \ifLineNumbers
    \let\mathenvironment\lneq
    \let\endmathenvironment\endlneq
  \else
    \let\mathenvironment\oldequation
    \let\endmathenvironment\endoldequation
  \fi 
  \begin{mathenvironment}}
  {\end{mathenvironment}}








\usepackage{titling}
%\pretitle{\begin{center}\LARGE}
%\posttitle{\par\end{center}\vskip 0em}
%\renewcommand{\maketitle}{\pretitle \title \posttitle}
%\keepthetitle

\preauthor{}
\postauthor{}
\author{}

\predate{}
\postdate{}
\date{}


\makeatletter
    \long\def\@author{\,}
    \long\def\@affil{\,}
    \long\def\@authorOne{\,}
    \long\def\@affilOne{\,}
    \long\def\@authorTwo{\,}        
    \long\def\@affilTwo{\,} 
    \long\def\twoauthors#1#2{}
    \long\def\twoaffiliations#1#2{}
    \long\def\threeauthors#1#2#3{}
    \long\def\threeaffiliations#1#2#3{}
    \long\def\fourauthors#1#2#3#4{} 
    \long\def\fouraffiliations#1#2#3#4{}
\makeatother



